Perfectly Undetectable Reflection and Scaling False Data Injection Attacks via Affine Transformation on Mobile Robot Trajectory Tracking Control

With the increasing integration of cyber-physical systems (CPS) into critical applications, ensuring their resilience against cyberattacks is paramount. A particularly concerning threat is the vulnerability of CPS to deceptive attacks that degrade system performance while remaining undetected. This paper investigates perfectly undetectable false data injection attacks (FDIAs) targeting the trajectory tracking control of a non-holonomic mobile robot. The proposed attack method utilizes affine transformations of intercepted signals, exploiting weaknesses inherent in the partially linear dynamic properties and symmetry of the nonlinear plant. The feasibility and potential impact of these attacks are validated through experiments using a Turtlebot 3 platform, highlighting the urgent need for sophisticated detection mechanisms and resilient control strategies to safeguard CPS against such threats. Furthermore, a novel approach for detection of these attacks called the state monitoring signature function (SMSF) is introduced. An example SMSF, a carefully designed function resilient to FDIA, is shown to be able to detect the presence of a FDIA through signatures based on systems states.

==> overflown.tex <==
%Cyber-physical systems (CPS) are often subject to deceptive cyberattacks designed not only to degrade system performance but also to remain undetectable. Understanding how such attacks can be deployed is crucial to developing resilient CPS. In this paper, we present a method for designing false data injection attacks (FDIAs) based on affine transformations of intercepted signals, utilizing only partial knowledge of a nonlinear dynamic plant. The paper derives conditions for the application of perfectly undetectable attacks on the trajectory tracking control of a non-holonomic mobile robot. Experimental results demonstrate that perfectly undetectable FDIAs, in the form of scaling and reflection, can be implemented in nonlinear systems by exploiting weaknesses such as symmetry and the partially linear dynamic properties of the nonlinear plant.
%Cyber-physical systems (CPS) are vulnerable to deceptive cyberattacks designed to degrade system performance while remaining undetectable.  This paper examines perfectly undetectable false data injection attacks (FDIAs) on the trajectory tracking control of a non-holonomic mobile robot.  The proposed attack method utilizes affine transformations of intercepted signals, exploiting weaknesses inherent in the partially linear dynamic properties and symmetry of the nonlinear plant.  The paper derives conditions for achieving perfectly undetectable attacks, demonstrating that coordinated manipulation of both control commands and observables can create the illusion of normal system operation, even when the actual robot behavior deviates significantly from the intended trajectory. Experimental results validate the feasibility of implementing these attacks in a real-world scenario using a Turtlebot 3 platform. These findings highlight the need for more robust security measures to protect CPS from increasingly sophisticated attack vectors.



%For example, 
%using PR, 
%\begin{equation}
%    \begin{split}
%$    \hat{\Phi}(x,y) =  \hat{\zeta}_0 + \hat{\zeta}_1x + \hat{\zeta}_2y + \hat{\zeta}_3x^2 + \hat{\zeta}_4xy + \hat{\zeta}_5y^2 + \hat{\zeta}_6x^3  + \h    X = rXnow.iloc[:,:]
%at{\zeta}_7x^2y + \hat{\zeta}_8xy^2 + \hat{\zeta}_9y^3 + \hat{\zeta}_{10}x^4 + \hat{\zeta}_{11}x^3y  + \hat{\zeta}_{12}x^2y^2 + \hat{\zeta}_{13}xy^3 + \hat{\zeta}_{14}y^4
%$
%\end{split}
%\end{equation}
%can be estimated
%\noindent
%by solving the least squares problem to find the coefficient vector $\hat{\bm{\zeta}}=[\hat{\zeta}_0, \hat{\zeta}_1, \cdots, ]^T$:
%    \begin{equation}
%$    \hat{\bm{\zeta}} = (\bm{X}^T \bm{X})^{-1}\bm{X}^T \bm{z}$
%    \end{equation}
%where $\bm{X}$ is the feature matrix for each data point $(x_i, y_i)$, $i=1, \cdots, N$, and its $i$-th row vector is given as:
%    \begin{equation}
%$    \bm{X}_i = [1, x_i, y_i, x_i^2, x_iy_i, y_i^2, x_i^3, x_i^2y_i, x_iy_i^2, y_i^3, x_i^4, x_i^3y_i, x_i^2y_i^2, x_iy_i^3, y_i^4]
%$ by assuming the attacker knows the degree of the polynomial
%    \end{equation}
%and the observed values $\bm{z}_i = \Phi(x_i, y_i)$ into a vector: 
%    \begin{equation}
%$    \bm{z} = [z_1, z_2, \ldots, z_N]^T
%$
%    \end{equation}
%Note that the coefficient vector $\hat{\bm{\zeta}}$ can be obtained using various regression techniques beyond ordinary least squares. 


% Results show that the number of data points along the trajectory is in general insufficient for the attacker to precisely estimate the signature function. 

% \begin{itemize}
%     \item {\bf Normal operation} (no attack):  
%     \item  {\bf Scenario 1 - Reflection attack} 
%     \item {\bf Scenario 2 - Scaling attack} 
% \end{itemize}


% Case 1: Polynomial regression.
% Along trajectory, 100, 200, 500 (by here experiments), (from here simulation) 1000, 2000, 5000 points
% No attack (simply see if the attacker can reproduce the same Phi)  MSE, R2
% Reflection MSE, R2
% Scaling MSE, R2
% Case 2: GPR
% The same as above



%Fig. \ref{exp_PhiScenarios} shows the performance of $\hat{\Phi}$ retroactively estimated through PR and GPR with 500 samples of the experimental data.
%It can be seen that accurate offline regression is achieved for the unattacked dataset as shown in Fig. \ref{exp_PhiScenarios}(a).  However, there are notable discrepancies between true values and estimated values in the reflected (b) and scaled (c) attack cases.
%Due to the nature of regression methods,  accuracy in extrapolation is difficult to achieve, generally since the $\Phi$ values for the reflected case is closer to the original $\Phi$, both regression methods performed better in the reflection case as can be seen in Fig. \ref{exp_PhiScenarios} (b).
%The performance of each regression method is evaluated in Fig. \ref{exp_metrics} and \ref{sim_metrics}. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Fig 14 shows the output of the signature function under two FDIA attack scenarios discussed in section above. Due to the FDIA to the input commands, the robot's position has been altered from the expected range.  If the controller can observe $\Phi(x)$ without any additional FDIA, the controller can detect the attack through comparing it with the expected values generated from the desired trajectory. A significant disparity is indicative of an attack on the system; this deviation is dependent on the attack parameters. 
  
%As shown in Fig 14 the scaling attack affects the $\Phi$ values more drastically as the magnitude of the robot’s position sees bigger change than the reflection function. If the signature function is constructed according to the standards of (section above) then constant matrices  
%$S_\Phi$ and $d_\Phi$  such that $S_\Phi \Phi(x) + d_\Phi = \Phi(\tilde x)$ does not exist. 

%An alternative for the attacker is then to attempt to perform estimation of $\Phi$ through collected data. 
%PR and GPR is performed with the scikit-learn library [REF]. $\Phi(x)$ and x values are used as labeled data for training. 
%The attacker is assumed to eavesdrop for the first 3 seconds of operation, and then uses the acquired $\hat \Phi$ to predict the following values. In this instance the attacker allows the controller to view $\Phi(x)$ before $t=3$ 
  
%Fig 15 shows the comparison between $\hat\Phi(\tilde x)$ and $\Phi(\tilde x)$ over time for two scenarios. Over the first three seconds the attacker can collect 150 sample points for regression, which is 10 times the VC dimension of (\ref{representativemonitoringfunction}). 
%However, as the sample is not distributed evenly within the target space, the estimation fails, and the security of the signature function holds. 
%In this instance, the attacker used a sample limited to the trajectory, leading to poorer estimations. 

% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=1\columnwidth]{figs/exp_PhiScenarios.eps}
% 	\caption{True $\bm{\Phi}$ values compared $\hat{\bm{\Phi}}$ acquired through PR and GPR with 500 samples for (a) original trajectory (b) reflection attack (c) scaling attack trajectory. }
% 	\label{exp_PhiScenarios}
% \end{figure}

%It should be emphasized that the function will lose all effectiveness if $\Phi(x)$ is exposed to or known by the attacker as attack $\bm{S_\Phi} = \bm{0}, \bm{d_\Phi} = \bm{\Phi}(\bm{x})$ can be used to bypass the signature function.

  % \item Condition 2 (observing the nominal dynamics): $\left. \frac{\partial \bm{\alpha} (\bm{x})}{\partial \bm{x}}\right|_{\bm{x}=\bm{\alpha}^{-1}(\bm{\tilde{x}})} \bm{f}(\bm{\alpha}^{-1}(\bm{\tilde{x}}))  + \bm{g}((\bm{\alpha}^{-1}(\bm{\tilde{x}})){\bm{\beta}(\bm{u})} = \bm{f}({\bm{x}'}) + \bm{g}({\bm{x}'}){\bm{u}}, \forall \bm{u}$ ensures that the compromised system's dynamics, as observed by the controller, is identical to the nominal (unattacked) system's dynamics for all possible inputs, $\bm{u}$.
